Rate Adaptation for Secure HARQ Protocols

This paper investigates the incremental-redundancy hybrid-automatic repeat request (IR-HARQ) transmission over independent block-fading channels in the presence of an eavesdropper, where the secrecy of the transmission is ensured via introduction of dummy-messages. Since the encoder only knows the statistics of the channel state, the secrecy and the reliability are defined in a probabilistic framework. Unlike previous works on this subject, we design a coding strategy tailored to IR-HARQ by splitting the dummy-message rate over several rate parameters. These additional degrees of freedom improve the match between the dummy-message rates and the realizations of the eavesdropper channels. We evaluate the performance in terms of secrecy outage probability, connection outage probability and throughput and we compare it with the benchmark paper by Tang et al. Numerical examples illustrate that, comparing to existing alternatives, splitting of the dummy-message rate provides higher throughput and lower expected duration/average delay.

==> Includes/DiscreteChannels.tex <==

%\newpage.
%\newpage

\section{An Intuition with Discrete Channel States}\label{sec:NumericalResults}


We consider the  scenario represented by Fig. \ref{fig:IndependentChannelb}, in which the channel states of the legitimate decoder and of the eavesdropper are discrete and uniformly distributed over $\{k^y,k'^y\}$ and $\{k^z,k'^z\}$. We assume  the connection and the secrecy outage  probability must be lower than $\xi_{\sf{c}}= 0.25$ and $ \xi_{\sf{s}}= 0.125$ for $L=2$ possible transmissions.
\begin{figure}[!h]
\begin{scriptsize}
\begin{center}
\psset{xunit=0.45cm,yunit=0.45cm}
\begin{pspicture}(0,-2.5)(16,8)
\rput[u](1,8){\textcolor[rgb]{0.0,0.0,1.0}{First Transmission}}
\psframe(0,0)(1,1)
\psframe(0,-2)(1,-1)
\psframe(6,0)(7,1)
\psframe(6,-2)(7,-1)
\psline[linewidth=1pt]{->}(1,0.5)(6,0.5)
\psline[linewidth=1pt]{->}(1,-1.5)(6,-1.5)
\rput[u](3.5,0.9){$I (X_1; Z_1|{k}^z_1) = 2$}
\rput[u](3.5,-0.7){$I (X_1; Z_1|{k}'^z_1) = 3.5$}
\rput(0.5,0.5){$\C$}
\rput(0.5,-1.5){$\C$}
\rput(6.5,0.5){$\mc{E}$}
\rput(6.5,-1.5){$\mc{E}$}
\rput(3,1.8){\textcolor[rgb]{1.0,0.0,0.0}{$\mc{P}(k^z_1) = \mc{P}(k'^z_1) = 1/2$}}
\psframe(0,5)(1,6)
\psframe(0,3)(1,4)
\psframe(6,5)(7,6)
\psframe(6,3)(7,4)
\psline[linewidth=1pt]{->}(1,5.5)(6,5.5)
\psline[linewidth=1pt]{->}(1,3.5)(6,3.5)
\rput[u](3.5,5.9){$I (X_1; Y_1|k^y_1) = 4$}
\rput[u](3.5,3.9){$I (X_1; Y_1|k'^y_1) = 5$}
\rput(0.5,5.5){$\C$}
\rput(0.5,3.5){$\C$}
\rput(6.5,5.5){$\D$}
\rput(6.5,3.5){$\D$}
\rput(3,6.8){\textcolor[rgb]{1.0,0.0,0.0}{$\mc{P}(k^y_1) = \mc{P}(k'^y_1) = 1/2$}}
\rput[u](12,8){\textcolor[rgb]{0.0,0.0,1.0}{Second Transmission}}
\psline[linewidth=1pt]{-}(8,-2)(8,8)
\psframe(10,0)(11,1)
\psframe(10,-2)(11,-1)
\psframe(16,0)(17,1)
\psframe(16,-2)(17,-1)
\psline[linewidth=1pt]{->}(11,0.5)(16,0.5)
\psline[linewidth=1pt]{->}(11,-1.5)(16,-1.5)
\rput[u](13.5,0.9){$I (X_2; Z_2|{k}^z_2) = 2$}
\rput[u](13.5,-0.7){$I (X_2; Z_2|{k}'^z_2) = 3.5$}
\rput(10.5,0.5){$\C$}
\rput(10.5,-1.5){$\C$}
\rput(16.5,0.5){$\mc{E}$}
\rput(16.5,-1.5){$\mc{E}$}
\rput(13,1.8){\textcolor[rgb]{1.0,0.0,0.0}{$\mc{P}(k^z_2) = \mc{P}(k'^z_2) = 1/2$}}
\psframe(10,5)(11,6)
\psframe(10,3)(11,4)
\psframe(16,5)(17,6)
\psframe(16,3)(17,4)
\psline[linewidth=1pt]{->}(11,5.5)(16,5.5)
\psline[linewidth=1pt]{->}(11,3.5)(16,3.5)
\rput[u](13.5,5.9){$I (X_2; Y_2|k^y_2) = 4$}
\rput[u](13.5,3.9){$I (X_2; Y_2|k'^y_{2}]) = 5$}
\rput(10.5,5.5){$\C$}
\rput(10.5,3.5){$\C$}
\rput(16.5,5.5){$\D$}
\rput(16.5,3.5){$\D$}
\rput(13,6.8){\textcolor[rgb]{1.0,0.0,0.0}{$\mc{P}(k^y_2) = \mc{P}(k'^y_2) = 1/2$}}
\end{pspicture}
\caption{In both transmissions, the capacity of the channel to the legitimate decoder takes two possible values $\{4 , 5 \}$ with probability $(1/2, 1/2)$ and the capacity of the channel to the eavesdropper takes two possible values $ \{2 , 3.5 \}$ with probability $(1/2, 1/2)$.}\label{fig:IndependentChannelb}
\end{center}
\end{scriptsize}
\end{figure}
%These values are rather large and this is due to the small number of possible transmissions $L=2$ and small cardinality of the set of channel states. 
We investigate the optimal performances of the ASR-code whose existence is stated in Theorem  \ref{theo:RandomLeszekCode} and we compare its performance to the coding schemes introduced in \cite{TangLiuSpasojevicPoor09} \textcolor[rgb]{0,0,1}{ and  in \cite{TomasinLaurenti14}.}

%, in which the dummy-message rate $ \textsf{R}_{2} = 0$ is zero. 


\subsection{Secure HARQ protocol of Tang et al. \cite{TangLiuSpasojevicPoor09}}

\textcolor[rgb]{0,0,1}{This protocol is a particular case of the ASR-code in which the dummy-message rate $ \textsf{R}_{2} = 0$ is zero. As depicted on fig. \ref{fig:RateRegionsPoor}, after $L=2$ transmissions, the decoding is correct if:
\begin{eqnarray}
\textsf{R} + \textsf{R}_1 &\leq&  I(X_1;Y_1|k_1) +  I(X_2;Y_2|k_2),
\end{eqnarray}
and the transmission is secret if:
\begin{eqnarray}
\textsf{R}_1 &\geq&  I(X_1;Y_1|k_1) +  I(X_2;Y_2|k_2).
\end{eqnarray}}
\begin{figure}[!ht]
\begin{center}
\psset{xunit=1cm,yunit=1cm}
\begin{pspicture}(-1,-1)(5,5)
\pspolygon*[linecolor=vertclair](0,3)(3,0)(5.5,0)(5.5,4.5)(0,4.5) 
\pspolygon*[linecolor=red](0,0)(0,1.5)(1.5,0)
\pspolygon[fillstyle=hlines,hatchcolor=blue,linecolor=white](3,0)(5.5,0)(5.5,4.85)(3,4.85)
\psline[linewidth=0.5pt]{->}(-1,0)(6,0)
\psline[linewidth=0.5pt]{->}(0,-1)(0,5)
\rput[d](5.5,-0.3){$I(X_1;Y_1|k_1)$}
\rput[d](5.5,-0.7){$I(X_1;Z_1|k_1)$}
\rput[r](-0.2,4.8){$I(X_2;Y_2|k_2)$}
\rput[r](-0.2,4.4){$I(X_2;Z_2|k_2)$}
\psline[linewidth=0.5pt,linestyle=dotted](0,3)(3,0)
\psdots(1.5,0)(3,0)(0,3)(0,1.5)
\rput[d](1.5,-0.3){$\textsf{R}_{1}$}
\rput[u](2,3.5){(D)}
\rput[u](0.5,0.5){(S)}
\rput[r](-0.2,1.5){$\textsf{R}_{1}$}
\rput[r](-0.2,3){$\textsf{R} + \textsf{R}_{1}$}
\psline[linewidth=0.5pt,linestyle=dotted](1.5,0)(0,1.5)
\psline[linewidth=1pt,linestyle=dashed,linecolor = blue](3,0)(3,5)
\rput[d](3,-0.3){ $\; \textsf{R} + \textsf{R}_{1}$}
\rput[l](3,5){ $\;\textcolor[rgb]{0.00,0.00,1.00}{\textsf{Ack}_1}$}
\rput[r](3,5){$ \textcolor[rgb]{0.00,0.00,1.00}{\textsf{Nack}_1} \;$ }
\end{pspicture}
\caption{Regions of correct decoding (D) and secret transmission (S) of Tang et al. \cite{TangLiuSpasojevicPoor09}.}\label{fig:RateRegionsPoor}
\end{center}
\end{figure}


%\newpage
\subsection{Secure HARQ protocol of Tomasin and Laurenti \cite{TomasinLaurenti14}}
\textcolor[rgb]{0,0,1}{This protocol, called S-HARQ in \cite[Sec. V]{TomasinLaurenti14}, is defined differently from the one of Tang et al. \cite{TangLiuSpasojevicPoor09} and from the ASR-code. Although it involves multiple dummy-message rates $(\textsf{R}_1 , \textsf{R}_2)$,  the regions of correct decoding: 
%As depicted on fig. \ref{fig:RateRegionsTomasin}, after $L=2$ transmissions, the decoding is correct if:
\begin{eqnarray}
\textsf{R} &\leq&  \max\Big(I(X_1;Y_1|k_1) -  \textsf{R}_1 , 0 \Big)  \nonumber \\
&+&   \max\Big(I(X_2;Y_2|k_2)  -  \textsf{R}_2 , 0\Big),
\end{eqnarray}
and secret transmission, depicted on fig. \ref{fig:RateRegionsTomasin} are different from the ones of fig. \ref{fig:RateRegions}, corresponding to ASR-code.
\begin{eqnarray}
\textsf{R}_1 \geq  I(X_1;Y_1|k_1) ,\qquad
\textsf{R}_2 \geq   I(X_2;Y_2|k_2).
\end{eqnarray}}
\begin{figure}[!ht]
\begin{center}
\psset{xunit=1cm,yunit=1cm}
\begin{pspicture}(-1,-1)(5,5.5)
\pspolygon*[linecolor=vertclair](0,2.5)(1.5,2.5)(3,1)(3,0)(5.5,0)(5.5,4.5)(0,4.5) 
\pspolygon*[linecolor=red](0,0)(0,1)(1.5,1)(1.5,0)
\pspolygon[fillstyle=hlines,hatchcolor=blue,linecolor=white](3,0)(5.5,0)(5.5,4.85)(3,4.85)
\psline[linewidth=0.5pt]{->}(-1,0)(6,0)
\psline[linewidth=0.5pt]{->}(0,-1)(0,5)
\rput[d](5.5,-0.3){$I(X_1;Y_1|k_1)$}
\rput[d](5.5,-0.7){$I(X_1;Z_1|k_1)$}
\rput[r](-0.2,5.4){$I(X_2;Y_2|k_2)$}
\rput[r](-0.2,5){$I(X_2;Z_2|k_2)$}
\psline[linewidth=0.5pt,linestyle=dotted](0,4)(4,0)
\psline[linewidth=0.5pt,linestyle=dotted](0,2.5)(5.5,2.5)
\psdots(1.5,0)(0,4)(0,1)(0,2.5)(3,0)
\rput[d](1.5,-0.3){$\textsf{R}_{1}$}
\rput[r](-0.2,1){$\textsf{R}_{2}$}
\rput[r](-0.2,2.5){$\textsf{R} + \textsf{R}_{2}$}
\rput[r](-0.2,4){$\textsf{R} + \textsf{R}_{1} + \textsf{R}_{2}$}
\psline[linewidth=0.5pt,linestyle=dotted](0,1)(5.5,1)
\psline[linewidth=0.5pt,linestyle=dotted](1.5,0)(1.5,4.5)
\psline[linewidth=0.5pt,linestyle=dotted](2.5,0)(0,2.5)
\psline[linewidth=1pt,linestyle=dashed,linecolor = blue](3,0)(3,5)
\rput[d](3,-0.3){ $\; \textsf{R} + \textsf{R}_{1}$}
\rput[l](3,5){ $\;\textcolor[rgb]{0.00,0.00,1.00}{\textsf{Ack}_1}$}
\rput[r](3,5){$ \textcolor[rgb]{0.00,0.00,1.00}{\textsf{Nack}_1} \;$ }
\rput[u](2,3.5){(D)}
\rput[u](0.5,0.5){(S)}
\end{pspicture}
\caption{Regions of correct decoding (D) and secret transmission (S) of Tomasin and Laurenti \cite{TomasinLaurenti14}.}
\label{fig:RateRegionsTomasin}
\end{center}
\end{figure}

\vspace{-0.5cm}

\subsection{Performance Comparison between ASR-code, \cite{TangLiuSpasojevicPoor09}, \cite{TomasinLaurenti14}}
\textcolor[rgb]{0,0,1}{Fig. \ref{fig:DiscreteChannelsThroughput_2017_05_16} compares the performances of the three protocols in terms of secrecy throughput $\eta$.%, Def. \ref{def:SecrecyThroughput}.
\begin{figure}[ht!]
\begin{scriptsize}
\psfragscanon
\psfrag{labelx}[][]{Secrecy Rate: $\textsf{R}$}
\psfrag{labely}[][]{Secrecy Throughput: $\eta$}
\psfrag{datadatadatadatadata1}[l][l]{ASR-code}
\psfrag{datadatadatadatadata2}[l][l]{Tang et al. \cite{TangLiuSpasojevicPoor09}}
\psfrag{datadatadatadatadata3}[l][l]{Tomasin  \cite{TomasinLaurenti14}}
\includegraphics[width=0.5\textwidth]{./figures/DiscreteChannelsThroughput_2017_05_16.eps}
\end{scriptsize}
\vspace{-0.9cm}
\caption{Secrecy throughput for $L=2$ possible transmissions and outage parameters $\xi_{\sf{c}}= 0.25$, $ \xi_{\sf{s}}= 0.125$.}\label{fig:DiscreteChannelsThroughput_2017_05_16}
\end{figure}
The ASR-code outperforms both protocols of Tang et al. \cite{TangLiuSpasojevicPoor09} and Tomasin and Laurenti \cite{TomasinLaurenti14} for the secrecy rate $\textsf{R}= 1.5$, dummy message rates $(\textsf{R}_1, \textsf{R}_2 ) = (3.5,2)$ and outage probabilities $(\mc{P}_{\sf{co}},\mc{P}_{\sf{so}} )= (0,0.125)$. \\
$\bullet$ For Tang et al. \cite{TangLiuSpasojevicPoor09}, the dummy-message rate $\textsf{R}_1^{\text{Tang et al.}} = 7$ corresponding to $L=2$ transmissions is high and prevents the first transmission to be decoded correctly. \\
$\bullet$ For Tomasin and Laurenti \cite{TomasinLaurenti14}, the second dummy-message rate $\textsf{R}_2^{\text{Tomasin}} = 3.5$ is higher than $\textsf{R}_2 =2$ for ASR-code. Hence, when the secrecy rate exceeds $\textsf{R}\geq 1.5$, the connection outage probability jumps to $\mc{P}_{\sf{co}}=0.25$ and reduces the secrecy throughput.}

\textcolor[rgb]{0,0,1}{For this example, the ASR-code provides more than $33,3\%$ of increase compared to the protocols of Tang et al. \cite{TangLiuSpasojevicPoor09} and Tomasin and Laurenti \cite{TomasinLaurenti14}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%
%%%%%% More Information About the Rates and Outages
%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{figure}[ht!]
%\begin{scriptsize}
%\psfragscanon
%\psfrag{labelx}[][]{Secrecy Rate: $\textsf{R}$}
%\psfrag{labely}[][]{Secrecy Throughput: $\eta$}
%\psfrag{datadatadatadatadata1}[l][l]{ASR-code}
%\psfrag{datadatadatadatadata2}[l][l]{Tang et al. \cite{TangLiuSpasojevicPoor09}}
%\psfrag{datadatadatadatadata3}[l][l]{Tomasin  \cite{TomasinLaurenti14}}
%\includegraphics[width=0.5\textwidth]{./figures/DiscreteChannelsRate_2017_05_16.eps}
%\end{scriptsize}
%\vspace{-0.9cm}
%\caption{Dummy-message rates for $L=2$ possible transmissions and outage parameters $\xi_{\sf{c}}= 0.25$, $ \xi_{\sf{s}}= 0.125$.}\label{fig:DiscreteChannelsRate_2017_05_16}
%\end{figure}
%
%
%\begin{figure}[ht!]
%\begin{scriptsize}
%\psfragscanon
%\psfrag{labelx}[][]{Secrecy Rate: $\textsf{R}$}
%\psfrag{labely}[][]{Secrecy Throughput: $\eta$}
%\psfrag{datadatadatadatadata1}[l][l]{ASR-code}
%\psfrag{datadatadatadatadata2}[l][l]{Tang et al. \cite{TangLiuSpasojevicPoor09}}
%\psfrag{datadatadatadatadata3}[l][l]{Tomasin  \cite{TomasinLaurenti14}}
%\includegraphics[width=0.5\textwidth]{./figures/DiscreteChannelsOutage_2017_05_16.eps}
%\end{scriptsize}
%\vspace{-0.9cm}
%\caption{Connection and secrecy outages for $L=2$ possible transmissions and outage parameters $\xi_{\sf{c}}= 0.25$, $ \xi_{\sf{s}}= 0.125$.}\label{fig:DiscreteChannelsOutage_2017_05_16}
%\end{figure}
%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









%\newpage
%
%
%
%\subsection{ASR-code with optimization over $\textsf{R}_{1}$ only}
%\begin{figure}[ht!]
%\centering
%\begin{minipage}{0.48\linewidth}
%\begin{scriptsize}
%\psfragscanon
%\psfrag{aa}[][l]{$\textsf{R}_2=0$}
%\psfrag{bb}[][]{
%\begin{picture}(0,0)
%\put(0.15, 0.2){\makebox(0,0)[c]{$\eta_0 = 1.125$}}
%\put(20,0){\vector(4,-3){10}}
%\end{picture}}
%\includegraphics[width=1\textwidth]{./figures/OptimalThroughputR2016_10_12.eps}
%\end{scriptsize}
%\vspace{-0.6cm}
%\caption{Throughput $\textcolor[rgb]{0.00,0.00,0.00}{\eta} $ optimized over  $\textcolor[rgb]{0.00,0.00,0.00}{\textsf{R}_{1}}$ depending  on the rate parameter $\textsf{R}$, with $ \textsf{R}_{2} =0 $.}\label{fig:LeszekCoding025125R2013_04_02}
% \end{minipage}\hfill
%\begin{minipage}{0.480\linewidth}
%\begin{scriptsize}
%\psfragscanon
%\psfrag{aa}[][l]{$\textsf{R}_2=0$}
%\psfrag{bb}[][]{
%\begin{picture}(0,0)
%\put(0.15, 0.2){\makebox(0,0)[c]{$\eta_0 = 1.125$}}
%\put(20,0){\vector(4,-3){10}}
%\end{picture}}
%\includegraphics[width=1\textwidth]{./figures/OptimalThroughputRW2016_10_12.eps}
%\end{scriptsize}
%\vspace{-0.6cm}
%\caption{Throughput $\textcolor[rgb]{0.00,0.00,0.00}{\eta} $ optimized over $\textsf{R}$ depending  on the rate parameter $\textcolor[rgb]{0.00,0.00,0.00}{\textsf{R}_{1}}$, with $ \textsf{R}_{2} = 0$.}\label{fig:LeszekCoding025125RW2013_04_02}
% \end{minipage}\hfill
%\end{figure}
%We consider the framework of \cite{TangLiuSpasojevicPoor09} where the second dummy-message rate is null $\textsf{R}_{2}=0$.  The optimal dummy-message rate $\textsf{R}^{\diamond}_{1}=6$ is high since  it must be adapted to two transmissions. This prevents the first transmission to be decoded correctly. Fig. \ref{fig:LeszekCoding025125R2013_04_02} and \ref{fig:LeszekCoding025125RW2013_04_02} show that  the optimal parameters are $(\textsf{R}^{\diamond}, \textsf{R}^{\diamond}_{1}) = (3,6)$. The probability of having a $\sf{NACK}_1$ feedback after the first transmission is equal to: $\mc{P}(\sf{NACK}_1)=1$. The  secrecy throughput is equal to 
%\begin{eqnarray}
%\eta =  \frac{3 \cdot (1 - 0.25) }{1 + 1 \cdot (1 - 0)} = \frac{9}{8} = 1.125. \label{eq:ThroughputPoor}
%\end{eqnarray}
%The secrecy outage has probability $\mc{P}_{\sf{so}} = 0$, since the dummy-message rate  $\textsf{R}^{\diamond}_{1} = 6$ is larger than the two best channels of the eavesdropper. The optimal secrecy rate is $\textsf{R}^{\diamond}=3$ and it induces a connection outage probability of $\mc{P}_{\sf{co}} =  0.25$.
%
%
%\subsection{ASR-code with optimization over both $\sf{R_1}$ and $\sf{R_2}$}
%
%The second dummy-message rate $ \textsf{R}_{2}$ provides an additional degree of freedom for the maximization of the secrecy throughput. 
%
%\begin{itemize}
%\item[$\bullet$] Fig. \ref{fig:OpimalThroughputRW2} shows that the  secrecy throughput is equal to $\textcolor[rgb]{0.00,0.00,0.00}{\eta} = 4/3 \simeq 1.333$ for a range of parameter $\textcolor[rgb]{0.00,0.00,0.00}{\textsf{R}_{2}^{\star}} \in [2,3]$. In this interval the secrecy outage probability $\mc{P}_{\sf{so}} \leq \xi_{\sf{s}}=1/8=0.125$ satisfies the constraint, the connection outage probability is equal to $\mc{P}_{\sf{co}} =0$ and $\mc{P}(\textsf{ACK}_1)=0.5$ stay constant. Hence the secrecy throughput is constant for $\textcolor[rgb]{0.00,0.00,0.00}{\textsf{R}_{2}^{\star}} \in [2,3]$.
%\item[$\bullet$] Fig. \ref{fig:OpimalParametersRW2} shows that the corresponding optimal parameters  are $(\textsf{R}^{\star} , \textsf{R}^{\star}_{1}) = (2,3)$. 
%\end{itemize}
%The secrecy outage probability is equal to $\mc{P}_{\sf{so}} = 1/8=0.125$ and the connection outage probability is equal to $\mc{P}_{\sf{co}} =  0$. 
% \begin{eqnarray}
%\eta =  \frac{2 \cdot (1 - 0) }{1 +  (1 - 0.5)} = \frac{4}{3} \simeq 1.333. \label{eq:ThroughputPoor}
%\end{eqnarray}
%The ASR-code allows to split the secrecy constraint over two parameters $(\textsf{R}^{\star}_1 , \textsf{R}^{\star}_{2}) = (3,2)$ instead of only $\textsf{R}^{\diamond}_{1} =6$. It induces a positive probability of decoding in the first transmission $\mc{P}(\textsf{ACK}_1)= 0.5$, that increases the secrecy throughput.
%
%\begin{figure}[ht!]
%%	\centering
%\begin{minipage}{0.48\linewidth}
%\begin{scriptsize}
%\psfragscanon
%\psfrag{aa}[][l]{$\textsf{R}_2=0$}
%\psfrag{bb}[][]{
%\begin{picture}(0,0)
%\put(0.15, 0.2){\makebox(0,0)[c]{$\eta_0 = 1.333$}}
%\put(20,0){\vector(4,-3){10}}
%\end{picture}}
%\includegraphics[width=1.1\textwidth]{./figures/OptimalThroughputRW2+_2016_10_12.eps}
%\end{scriptsize}
%\vspace{-0.7cm}
%\caption{Secrecy throughput $\textcolor[rgb]{0.00,0.00,0.00}{\eta} $ with optimal $(\textsf{R}^{\star}, \textsf{R}^{\star}_{1} )$ depending on  $\textsf{R}_{2}$.}\label{fig:OpimalThroughputRW2}
% \end{minipage}\hfill
%\begin{minipage}{0.48\linewidth}
%\begin{scriptsize}
%\psfragscanon
%\psfrag{aa}[][l]{$\textsf{R}_2=0$}
%\psfrag{bb}[][]{
%\begin{picture}(0,0)
%\put(0.15, 0.2){\makebox(0,0)[c]{$\eta_0 = 1.125$}}
%\put(20,0){\vector(4,-3){10}}
%\end{picture}}
%\includegraphics[width=1.1\textwidth]{./figures/OptimalParametersRW2+_2016_10_12.eps}
%\end{scriptsize}
%\vspace{-0.7cm}
%\caption{Optimal  $(\textsf{R}^{\star}, \textsf{R}^{\star}_{1})$ depending on  $\textsf{R}_{2}$.}\label{fig:OpimalParametersRW2}
% \end{minipage}
% \end{figure}
% For this example described by Fig. \ref{fig:IndependentChannelb}, the ASR-code provides more than $18,5\%$ of increase compared to the approach of  \cite{TangLiuSpasojevicPoor09}, with a  secrecy rate $\textsf{R}^{\star}=2$ lower than $\textsf{R}^{\diamond}=3$.
% 
% 
